Learning Locally, Revising Globally: Global Reviser for Federated Learning with Noisy Labels

Conventional federated learning (FL) heavily depends on high-quality labels, which are often impractical in the real world, leading to the federated label-noise (F-LN) problem. Worse still, the F-LN problem is exacerbated by the heterogeneity of FL, whereas clients experience different label-noise types, ratios, and data distribution. In this study, we first observe an intriguing phenomenon that the global model of FL exhibits a slow memorization of noisy labels, suggesting its ability to maintain reliable predictions and robust representations in FL. Motivated by this, we propose a novel method termed Federated Global Reviser (\method), a straightforward yet effective method comprising three modules that collaboratively rectify noisy labels and regularize local training. By exploiting this inherent property, \method\ improves the label-noise robustness of FL in a self-contained manner. Extensive experiments on three widely used F-LN benchmarks demonstrate the superior performance of FedGR, consistently outperforming eight state-of-the-art baselines even in severe label-noise and data heterogeneity. Code: https://github.com/cs-yuxintian/FedGR-ICML26

==> figs/ema.tex <==
% \begin{figure}[htpb!]
\begin{wrapfigure}{r}{0.52\textwidth}
    \centering
	\resizebox{0.5\textwidth}{!}{%
	\tikzset{every picture/.style={line width=0.75pt}} %set default line width to 0.75pt        
	
	\begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-1,xscale=1]
	%uncomment if require: \path (0,300); %set diagram left start at 0, and has height of 300
	
	%Straight Lines [id:da23814455082762354] 
	\draw    (47,32) -- (93.18,53.17) ;
	\draw [shift={(95,54)}, rotate = 204.62] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
	%Straight Lines [id:da7948655555116478] 
	\draw    (150,58) -- (196,58) ;
	\draw [shift={(198,58)}, rotate = 180] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
	%Straight Lines [id:da02483021552413045] 
	\draw    (343,58) -- (389,58) ;
	\draw [shift={(391,58)}, rotate = 180] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
	%Straight Lines [id:da013861871635753698] 
	\draw    (47,57) -- (93,57) ;
	\draw [shift={(95,57)}, rotate = 180] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
	%Shape: Brace [id:dp952853913522741] 
	\draw   (19,87) .. controls (19,91.67) and (21.33,94) .. (26,94) -- (59,94) .. controls (65.67,94) and (69,96.33) .. (69,101) .. controls (69,96.33) and (72.33,94) .. (79,94)(76,94) -- (112,94) .. controls (116.67,94) and (119,91.67) .. (119,87) ;
	%Shape: Brace [id:dp6735988092019111] 
	\draw   (127,87) .. controls (127,91.67) and (129.33,94) .. (134,94) -- (264,94) .. controls (270.67,94) and (274,96.33) .. (274,101) .. controls (274,96.33) and (277.33,94) .. (284,94)(281,94) -- (414,94) .. controls (418.67,94) and (421,91.67) .. (421,87) ;
	%Straight Lines [id:da33277273675495167] 
	\draw    (234,58) -- (280,58) ;
	\draw [shift={(282,58)}, rotate = 180] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
	%Straight Lines [id:da2642167484803609] 
	\draw    (343,33) -- (389.18,54.17) ;
	\draw [shift={(391,55)}, rotate = 204.62] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
	
	
	% Text Node
	\draw (1,45.4) node [anchor=north west][inner sep=0.75pt]    {$\mathbf{w}_{k,\ ema}^{t-1}$};
	% Text Node
	\draw (1,15.4) node [anchor=north west][inner sep=0.75pt]    {$\mathbf{w}_{g}^{t-1}$};
	% Text Node
	\draw (100,45.4) node [anchor=north west][inner sep=0.75pt]    {$\mathbf{w}_{k,\ ema}^{t,\ 0}$};
	% Text Node
	\draw (398,45.4) node [anchor=north west][inner sep=0.75pt]    {$\mathbf{w}_{k,\ ema}^{t,\ m_{k}}$};
	% Text Node
	\draw (205,49.4) node [anchor=north west][inner sep=0.75pt]    {$\cdots$};
	% Text Node
	\draw (60,21.4) node [anchor=north west][inner sep=0.75pt]    {$1-\gamma _{g}$};
	% Text Node
	\draw (162,65.4) node [anchor=north west][inner sep=0.75pt]    {$\gamma _{l}$};
	% Text Node
	\draw (356,66.4) node [anchor=north west][inner sep=0.75pt]    {$\gamma _{l}$};
	% Text Node
	\draw (61,64.4) node [anchor=north west][inner sep=0.75pt]    {$\gamma _{g}$};
	% Text Node
	\draw (0,108) node [anchor=north west][inner sep=0.75pt]   [align=left] {{\fontfamily{ptm}\selectfont {\small Globally Revised EMA Step}}};
	% Text Node
	\draw (223,108) node [anchor=north west][inner sep=0.75pt]   [align=left] {{\fontfamily{ptm}\selectfont {\small Usual Local EMA Step}}};
	% Text Node
	\draw (247,66.4) node [anchor=north west][inner sep=0.75pt]    {$\gamma _{l}$};
	% Text Node
	\draw (286,42.4) node [anchor=north west][inner sep=0.75pt]    {$\mathbf{w}_{k,\ ema}^{t,\ m_{k} -1}$};
	% Text Node
	\draw (286,12.4) node [anchor=north west][inner sep=0.75pt]    {$\mathbf{w}_{k}^{t,\ m_{k} -1}$};
	% Text Node
	\draw (357,22.4) node [anchor=north west][inner sep=0.75pt]    {$1-\gamma _{l}$};
	\end{tikzpicture}
	}
    \caption{\textcolor{blue}{Global model revised EMA update: The local EMA model, firstly revised by the global model with momentum decay $\gamma_g$, then undergoes its standard EMA update with momentum decay $\gamma_l$ on client $k$ at round $t$.}}
    \label{fig:local-ema-update}
% \end{figure}
\end{wrapfigure}
